diBELLA: Distributed Long Read to Long Read Alignment

We present a parallel algorithm and scalable implementation for genome analysis, specifically the problem of finding overlaps and alignments for data from "third generation" long read sequencers. While long sequences of DNA offer enormous advantages for biological analysis and insight, current long read sequencing instruments have high error rates and therefore require different approaches to analysis than their short read counterparts. Our work focuses on an efficient distributed-memory parallelization of an accurate single-node algorithm for overlapping and aligning long reads. We achieve scalability of this irregular algorithm by addressing the competing issues of increasing parallelism, minimizing communication, constraining the memory footprint, and ensuring good load balance. The resulting application, diBELLA, is the first distributed memory overlapper and aligner specifically designed for long reads and parallel scalability. We describe and present analyses for high level design trade-offs and conduct an extensive empirical analysis that compares performance characteristics across state-of-the-art HPC systems as well as a commercial cloud architectures, highlighting the advantages of state-of-the-art network technologies.

==> kmeranalysis.tex <==
%\section{Distributed \kmer Analysis}\label{sec:kmer_analysis}
%The first two stages together constitute \kmer Analysis, and computes a (global) histogram of the \kmers from the uniformly distributed input reads. The histogram is used to filter \kmers outside the reliable \kmer frequency range. Optionally, the full histogram is also provided to the user for independent analysis. The histogram computation primarily relies on two distributed data structures, a Bloom Filter and a hash table; these are described further in sections \ref{sec:bf} and \ref{sec:ht} respectively.

%%%%%%%%%%%%%%%%%%%%
%  BLOOM FILTER CONSTRUCTION %
%%%%%%%%%%%%%%%%%%%%
\section{Bloom Filter} \label{sec:bf} 
Singleton \kmers (\kmers occurring only once in the input) constitute the majority of the \kmer data set (up to $\approx$98\% from empirical observation) and further are not useful for detecting pairs of reads related by a common \kmer. Storing singletons is prohibitively expensive with respect to memory, since it would be $k$ times larger than the input size. Therefore the goal of this stage is to build a distributed Bloom filter to identify (with high probability) those \kmers that appears only once in the input and can therefore be ignored.  A bloom filter is an array of bits that uses multiple hash functions on each element to set bits in the array.  Due to collisions, a value may not be in the array even if its hash bits are set, but value with at least one 0 is guaranteed to not be in the set~\cite{bloomfilter}.  

Detecting singletons requires global information; a \kmer occurring only once in a partition of the input may or may not occur again in other partitions. We detect and avoid storing singletons by employing a Distributed Bloom Filter ~\cite{egeorganas2016}. Minimizing the Bloom Filter false positive rate depends on the (unknown \apriori) cardinality of the \kmer set. We approximate it using equation~\ref{eq:kmer_cardinality} and typical ratios of singleton \kmers to all \kmers across data sets. This provides fast and sufficiently accurate estimates, such that for data sets explored thus far, we have found more sophisticated cardinality estimation algorithms not worth the overhead. However, we employ the simple calculation only in load balancing and initializing the \kmer data structures.

We  follow the ideas and use code from the HipMer short read assembler~\cite{georganas2016} for this stage. The input reads are distributed roughly uniformly over the parallel processors (ranks) using parallel I/O. There are no guarantees about the order of the reads in the input (FASTQ) files, so nothing can be assumed about locality of reads. For load balancing, each rank parses its reads into \kmers, hashes the \kmer, and sends it to a processor indicated by the hash function. On the remote node, the \kmer will be inserted into its local Bloom filter. All of these $G \cdot d$ \kmers will be computed, and most will be communicated remotely, but the computation in this stage proceeds in phases with only a subset that fits in memory (and in outgoing communication buffers) at each phase. Once the hash table is initialized with these keys, the Bloom Filter can be freed. 

The Bloom filter is very effective on long read data with its high error rates, because there are so many (erroneous) singleton \kmers---up to $\approx98\%$ in practice.  Assuming $s$ phases, the cost of this bloom filter stage is: 

\begin{table}
\begin{tabular}{|r|l|}
  \hline
  computation per rank & $O(G \cdot d \ P)$ hashes \\  \hline
  communication volume per rank & $O(G \cdot d \cdot k \cdot (P-1)/P^2)$ \\ \hline
  number of messages per rank & $O(s \cdot (P-1))$ \\   \hline
  memory footprint per rank & $O(G \cdot d \cdot k / (P \cdot s)$ \\  \hline
\end{tabular}
\end{table}

The Bloom filter construction requires communicating nearly all (roughly $(P-1)/P$) of the \kmer instances to other processors, so $G*d*k * (P-1)/P$ characters in aggregate.   They are exchanged in bulk synchronous phases and inserted into Bloom Filter partitions at the destination. Those detected by the Bloom Filter to have occurred more than once are then also stored in the local hash table partition. Once the hash table is initialized with these keys, the Bloom Filter can be freed.

Figure \ref{fig:bf_efficiency} shows the efficiency of this stage on a 32 node AWS cluster, and is further discussed in the context of overall pipeline performance in Section~\ref{sec:performance}. The \lplabel (hashing and storing \kmers) speeds-up super-linearly, since more of the input fits in nearby memory as we scale the number of parallel processors. Each unit of data (\kmer) is represented with the number of bits equal to the nearest power of two larger than $k$. On the other hand, the {\it Exchange} efficiency, computed over the single (intra)node communication efficiency, degrades as expected, rapidly. Still, the overall efficiency, determined by both, remains high to 8 nodes and tails-off at 16-32 nodes (256-512 cores). %TODO highlight that the bloom filter exchange load is the second smallest and most uniform of the application exchanges

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/bf_efficiency}
  \caption{AWS Distributed Bloom Filter Strong Scaling Efficiency. Percent efficiency (log-scaled) calculated relative to the minimum number of nodes (1) is shown on the (y-axis). The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per core. Measurements were taken on an Amazon Web Services c3.8xlarge cluster of 32 nodes within in the same ``Placement Group". (Formatting to be updated for final.)}%
  \label{fig:bf_efficiency}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/titan_bf_efficiency}
  \caption{XK7 Distributed Bloom Filter Strong Scaling Efficiency. (Formatting to be updated for final.) Percent efficiency (log-scaled) calculated relative to the minimum number of nodes (1) is shown on the (y-axis). The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per L1 cache. Measurements were taken on a Cray XK7 within a 32 node allocation.}%
  \label{fig:titan_bf_efficiency}
\end{figure}

%%%%%%%%%%%%%%%%%%%
%  HASH TABLE CONSTRUCTION %
%%%%%%%%%%%%%%%%%%%

% Kathy's overview additions:
% This again communicates $P-1/P$ of the \kmers in the input, but also communicates and stores information about the read (an ID) and location of the \kmer instance within that read.

\section{Hash Table Construction}\label{sec:ht}
\Marquita{TODO: merge the following two paragraphs}
The goal of the second stage is to build a hash table with \kmers as keys and the read ID and position of the \kmer has a value.  The table will only store ``useful'' \kmers, i.e., those that appear between 2 and $m$ times in the input data set.  

In order to filter \kmers by their (global) frequency (with upper and lower limits), without \apriori information on the distribution of the \kmers in the input reads, we construct a distributed hash table mapping \kmers to their frequencies. Further, since our end goal is not simply to count and filter the \kmers, \Marquita{should we cite tools that do just k-mer counting like jellyfish to further highlight that this difference is important or leave it?} but rather also to compute all pairs of (reads) that share a retained \kmer, the hash table entries also contain the source locations of the \kmers. Source locations are defined by read identifiers and corresponding start indices of the \kmers within the reads. 
\Marquita{TODO: merge the above two paragraphs}

\Marquita{TODO: merge the following paragraphs, see next comments}
As in the previous stage, the \kmers are parsed from the input reads, hashed, and sent to the rank indicated by the hash function.  This is again done in memory-limited set of bulk-synchronous phases, but in this case the read ID and position within the read are communicated along with the \kmer.  

Once the data is exchanged, each rank checks the Bloom filter to see if each \kmer is in the Bloom filter, and if so, it adds the \kmer and associated information to the hash table.  Multiple read/positions are kept in a list associated with each \kmer, up to at most $m$.

After construction, any \kmers with frequency 1 or greater than $m$ are removed from the hash table.  

\Marquita{----TODO: merge the above paragraphs with the following paragraph----}

The distributed hash table is initialized as follows. The \kmers are parsed from the input reads, the reads having been partitioned uniformly over the parallel processors (ranks). Each rank buffers the entries that hash to remote locations in distributed memory until buffer limits are met. Then, the entries are communicated in a bulk synchronous many-to-many exchange. Once the data is exchanged, each rank updates its local partition of the distributed hash table with the received entries. All coalescing and counting is performed at the destination. Noting that location information will only be utilized for retained \kmers (those occurring at frequencies within the reliable \kmer range), we store no more locations per \kmer than the maximum reliable \kmer frequency. During the coalescing process, we might discover more locations than this for a given \kmer, but these \kmers and therefore their locations will never be used and are thus ignored. Finally, depending on the size of the input and memory and communication limits, it may take multiple rounds to read and exchange all the data. At the end of all exchanges, when each rank has complete (global) histogram information for its partition of the \kmer set, the histogram and related data is optionally output in parallel for the user. Lastly, \kmers that skipped the Bloom Filter and those exceeding the \kmer frequency threshold are removed from the hash table in a parallel traversal. 
\Marquita{TODO: merge the above paragraphs}

Figure~\ref{fig:ht_efficiency} shows the efficiency of this stage on a 32 node AWS cluster, and is further discussed in the context of overall pipeline performance in Section~\ref{sec:performance}. Like the \bfstage, \lplabel (\kmer hashing and storing with metadata) speeds-up super linearly. The exchange gets higher bandwidth utilization from sending the metadata along with the \kmers but still degrades as expected. The \overlabel efficiency again, is determined by both the \lplabel and \exchlabel efficiencies, and tails-off at 32 nodes (512 cores).

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/ht_efficiency}
  \caption{AWS Distributed Hash Table Construction Strong Scaling Efficiency. (Formatting to be updated for final.) Percent efficiency (log-scaled) calculated relative to the minimum number of nodes (1) is shown on the (y-axis). The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per core. Measurements were taken on an Amazon Web Services c3.8xlarge cluster of 32 nodes within in the same ``Placement Group".}%
  \label{fig:ht_efficiency}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/titan_ht_efficiency}
  \caption{XK7 Distributed Hash Table Construction Strong Scaling Efficiency. (Formatting to be updated for final.) Percent efficiency (log-scaled) calculated relative to the minimum number of nodes (1) is shown on the (y-axis). The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per L1 cache. Measurements were taken on a Cray XK7 within a 32 node allocation.}%
  \label{fig:titan_ht_efficiency}
\end{figure}


==> results.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/pipeline_efficiency}
  \caption{AWS Overall Pipeline Strong Scaling Efficiency. (Formatting to be updated for final.) The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per core. Percent strong scaling efficiency (log-scaled), relative to the minimum number of nodes (1 with 16 MPI ranks) is shown on the (y-axis). Measurements were taken on an Amazon Web Services c3.8xlarge cluster of 32 nodes within in the same ``Placement Group". }%
  \label{fig:pipeline_efficiency}
\end{figure}

%\iffalse %if we choose to include these results we can uncomment
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=\linewidth]{./figures/edison_pipeline_efficiency}
%  \caption{Cray XC30 Overall Pipeline Strong Scaling Efficiency. (Formatting to be updated for final.) The (x-axis) is the number of nodes, with 24 MPI ranks per node, 1 per core. Percent strong scaling efficiency (log-scaled), relative to the minimum number of nodes (1 with 24 MPI ranks) is shown on the (y-axis). Measurements were taken on a Cray XC30 with a Cray Aries interconnect, within a 32 node allocation (for comparison with AWS results). }%
%   \label{fig:edison_pipeline_efficiency}
%\end{figure}
%\fi

\begin{figure}[h]
  \centering 
  \includegraphics[width=\linewidth]{./figures/corih_pipeline_efficiency}
  \caption{Cray XC40 Overall Pipeline Strong Scaling Efficiency. (Formatting to be updated for final.) The (x-axis) is the number of nodes, with 32 MPI ranks per node, 1 per core. Percent strong scaling efficiency (log-scaled), relative to the minimum number of nodes (1 with 32 MPI ranks) is shown on the (y-axis). Measurements were taken on a Cray XC40 with a Cray Aries interconnect, within a 32 node allocation (for comparison with AWS results). }%
  \label{fig:corih_pipeline_efficiency}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/titan_pipeline_efficiency}
  \caption{Cray XK7 Overall Pipeline Strong Scaling Efficiency. (Formatting to be updated for final.) The (x-axis) is the number of nodes, with 16 MPI ranks per node. Percent strong scaling efficiency (log-scaled), relative to the minimum number of nodes (1 with 16 MPI ranks) is shown on the (y-axis). Measurements were taken on a Cray XK7 with a Cray Gemini interconnect, within a 32 node allocation (for comparison with AWS results). }%
  \label{fig:titan_pipeline_efficiency}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/corih_stage_pct_fine}
  \caption{Cray XC40 Pipeline Strong Scaling, Percent Overall Time by Stage. (Formatting to be updated...) The (x-axis) is the number of nodes, with 32 MPI ranks per node, 1 per core. The (y-axis) is percentage of total runtime (0-100\%). Measurements were taken on a Cray XC40 with a Cray Aries interconnect, within a 32 node allocation (for comparison with AWS results).}%
  \label{fig:cori_pct_runtime}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/titan_stage_pct_fine}
  \caption{Cray XK7 Pipeline Strong Scaling, Percent Overall Time by Stage. (Formatting to be updated...) The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per L1 cache. The (y-axis) is percentage of total runtime (0-100\%). Measurements were taken on a Cray XK7 with a Cray Gemini interconnect, within a 32 node allocation (for comparison with AWS results).}%
  \label{fig:titan_pct_runtime}
\end{figure}

\pagebreak %TODO remove after formatting fix
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{./figures/stage_pct_fine}
  \caption{AWS Pipeline Strong Scaling, Percent Overall Time by Stage. (Formatting to be updated...) The (x-axis) is the number of nodes, with 16 MPI ranks per node, 1 per core. The (y-axis) is percentage of total runtime. Measurements were taken on an Amazon Web Services c3.8xlarge cluster of 32 nodes within in the same ``Placement Group". }%
  \label{fig:pct_runtime}
\end{figure}
\pagebreak

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figures/cross_hpc_network}
  \caption{Overall vs. Exchanging Strong Scaling Efficiency across HPC Machines. (Formatting to be updated for final.) The (x-axis) is the number of nodes. Strong scaling efficiency (log-scaled), relative to the minimum number of nodes is shown on the (y-axis). Both overall (solid lines) and exchanging (dashed lines) efficiencies are shown. Measurements were taken on a Cray XK7 (Gemini), Cray XC40 (Aries), and Cray XC30 (Aries). The number of MPI Ranks per node was set equal to the number of cores ({\it Integer Cores} or L1 Caches w.r.t. Cray XK7) per node (16, 32, and 24, respectively). Each series was run within a 32 node allocation for comparison with AWS results.}%
  \label{fig:cross_hpc_network}
\end{figure}


